Harnessing Webpage UIs for Text-Rich Visual Understanding

Text-rich visual understanding-the ability to process environments where dense textual content is integrated with visuals-is crucial for multimodal large language models (MLLMs) to interact effectively with structured environments. To enhance this capability, we propose synthesizing general multimodal instructions from webpage UIs using text-based large language models (LLMs). Despite lacking direct visual input, text-based LLMs are able to process structured text representations from webpage accessibility trees. These instructions are then paired with UI screenshots to train multimodal models. We introduce MultiUI, a dataset containing 7.3 million samples from 1 million websites, covering diverse multimodal tasks and UI layouts. Models trained on MultiUI not only excel in web UI tasks-achieving up to a 48% improvement on VisualWebBench and a 19.1% boost in element accuracy on a web agent dataset Mind2Web-but also generalize surprisingly well to non-web UI tasks and even to non-UI domains, such as document understanding, OCR, and chart interpretation. These results highlight the broad applicability of web UI data for advancing text-rich visual understanding across various scenarios.

==> tables/ablation_task_type.tex <==
% \begin{table}[]
% \centering
% \small
% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
%  & \textbf{\makecell[c]{GUI\\Understanding}} & \textbf{\makecell[c]{GUI\\Grounding}} & \textbf{\makecell[c]{General OCR/\\DocVQA/ChartQA}} & \textbf{\makecell[c]{General\\Grounding}} & \textbf{All} \\
% \midrule
% \textbf{QA}        & 7.7   & 1.3  & 5.9  & -3.2 & 2.9  \\
% \textbf{Caption}   & 11.8  & -0.6 & 6    & -2   & 3.8  \\
% \textbf{OCR}       & 10.4  & 1.3  & 2.3  & 2.9  & 4.2  \\
% \textbf{Grounding} & -10.8 & 42.6 & -0.9 & 34.2 & 16.3 \\
% \bottomrule
% \end{tabular}}
% \caption{Ablation study of four task types. }
% \label{tab:ablation_task_type}
% \end{table}

\begin{table}[]
\centering
\small
    \resizebox{\textwidth}{!}{
        \begin{tabular}{cccccccccc}
            \toprule
                 & \multicolumn{2}{c}{\textbf{GUI Understanding}} & \multicolumn{2}{c}{\textbf{GUI Grounding}} & \multicolumn{2}{c}{\textbf{\makecell[c]{General OCR /\\DocQA / ChartQA}}} & \textbf{\makecell[c]{General\\Grounding}} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
                 & \makecell[c]{Visual\\WebBench}         & WebSRC         & SSpot(REC)         & RefExp         & DocVQA                   & ChartQA                  & \makecell[c]{RefCOCO+\\(REC)}      \\
            \midrule
            \textbf{QA}        & 16.4 & 11.1 & 7    & 8.5  & 8.2 & 5.4  & 5.1  \\
    \textbf{Caption}   & 9.5  & 7.1  & -0.7 & 0.4  & 5.4 & 4.4  & 3.7  \\
    \textbf{OCR}       & 15.3 & 2    & 0.6  & 0.4  & 2.7 & 2.9  & 3.5  \\
    \textbf{Grounding} & 1.4  & -8.6 & 50.9 & 39.5 & 1.9 & -1.1 & -0.6 \\
            \bottomrule
        \end{tabular}
    }
    
% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{ccccccc}{
% \toprule
% \multicolumn{2}{c}{\textbf{GUI Understanding}} & \multicolumn{2}{c}{\textbf{GUI Grounding}} & \multicolumn{2}{c}{\textbf{\makecell[c]{General OCR /\\DocQA / ChartQA}}} & \textbf{General Grounding} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
%              & \makecell[c]{Visual\\WebBench}         & WebSRC         & SSpot(REC)         & RefExp         & DocVQA                   & ChartQA                  & RefCOCO+(REC)      \\
% \midrule

% \bottomrule
% \end{tabular}}
\caption{Ablation study of four task types. }
\label{tab:ablation_task_type}
\end{table}

==> tables/grounding.tex <==

\begin{table}[t]
\centering
\small
% \tabcolsep=3pt
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\makecell[c]{\\ \textbf{Model}}} & \multicolumn{5}{c}{\textbf{GUI Grounding}} & \multicolumn{2}{c}{\textbf{General Grounding}} \\
\cmidrule(l){2-6} \cmidrule(l){7-8}
& \makecell[c]{VWB\\E-Ground$^*$} & \makecell[c]{VWB\\A-Ground$^*$} & \makecell[c]{ScreenSpot\\(REC)} & \makecell[c]{ScreenSpot\\(REG)} & RefExp & \makecell[c]{RefCOCO+\\(REC)} & \makecell[c]{RefCOCO+\\(REG)} \\
\midrule
GPT-4o \\
Claude 3.5 Sonnet \\
Pix2Struct \\
CogAgent \\
\midrule
\multicolumn{8}{c}{\textbf{Trained with only LLaVA-1.5 data}} \\
\midrule
LLaVA-1.5-7B \\
LLaVA-1.5-13B \\
LLaVA-Vicuna$^\dagger$ & 0.0 & 0.0 & 1.3 & 0.3 & 1.2 & 61.7 & 0.4 \\
\midrule
\multicolumn{8}{c}{Trained with LLaVA-1.5 data + \data{}} \\
\midrule
\model{}-Vicuna & 55.5 & 26.7 & 44.7 & 0.7 & 35.8 & 65.7 & 0.4 \\
\rowcolor{LightCyan} 
$\Delta$ over LLaVA-Vicuna & +55.5 & +26.7 & +43.4 & +0.4 & +34.6 & +4.0 & 0.0 \\
\midrule

\multicolumn{8}{c}{\textbf{Trained with only LLaVA-1.6 data}} \\
\midrule
LLaVA-1.6-7B \\
LLaVA-1.6-13B \\
LLaVA-1.6-34B \\
LLaVA-NeXT-8B \\
LLaVA-Llama3.1$^\dagger$ & 0.5 & 0.0 &  &  & 0.9 & 74.8 & 0.3 \\
LLaVA-Qwen2$^\dagger$ & 1.2 & 0.0 & 1.3 & 0.6 & 1.9 & 75.9 & 0.3 \\
\midrule
\multicolumn{8}{c}{Trained with LLaVA-1.6 data + \data{}} \\
\midrule
\model{}-Llama3.1 & 16.2 & 11.9 &  &  & 17.9 & 71.7 & 0.3  \\
\rowcolor{LightCyan} 
$\Delta$ over LLaVA-Llama3.1 & +16.2 & +11.9 &  &  & +17.0 & -3.1 & 0.0 \\
\midrule
\model{}-Qwen2 & 66.1 & 35.6 & 55.2 & 1.0 & 43.5 & 79.1 & 0.4 \\
\rowcolor{LightCyan} 
$\Delta$ over LLaVA-Qwen2 & +64.9 & +35.6 & +53.9 & +0.4 & +41.6 & +3.2 & +0.1 \\
\bottomrule
\end{tabular}
}
\caption{Results on multimodal grounding benchmarks.}
\label{tab:ground_exp}
\end{table}


==> tables/two_stage_training.tex <==

% \begin{table}[]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccccccc}
%         \toprule
%              & \multicolumn{2}{c}{\textbf{GUI Understanding}} & \multicolumn{2}{c}{\textbf{GUI Grounding}} & \multicolumn{2}{c}{\textbf{\makecell[c]{General OCR /\\DocQA / ChartQA}}} & \textbf{General Grounding} & \multicolumn{2}{c}{\textbf{General}} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10}
%              & \makecell[c]{Visual\\WebBench}         & WebSRC         & SSpot(REC)         & RefExp         & DocVQA                   & ChartQA                  & RefCOCO+(REC)       & MMBench         & MME            \\
%         \midrule
%         Single-stage & 75.4                        & 80.1               & 53                      & 43.2               & 83.7                         & 74.2                          & 74.5                         & 76.8                 & 1883.1             \\
% Two-stage    & 75.9                        & 82.9               & 55.2                    & 43.5               & 85.3                         & 74                            & 79.1                         & 77.4                 & 1905.1            \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Comparison between single-stage and two-stage training. }
%     \label{tab:two_stage_training}
% \end{table}


\begin{table}[]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccccccc}
        \toprule
             & \multicolumn{2}{c}{\textbf{GUI Understanding}} & \multicolumn{2}{c}{\textbf{GUI Grounding}} & \multicolumn{2}{c}{\textbf{\makecell[c]{General OCR /\\DocQA / ChartQA}}} & \textbf{\makecell[c]{General\\Grounding}} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
                 & \makecell[c]{Visual\\WebBench}         & WebSRC         & SSpot(REC)         & RefExp         & DocVQA                   & ChartQA                  & \makecell[c]{RefCOCO+\\(REC)}      \\
        \midrule
        \textbf{Single-stage} & 75.4                        & 80.1               & 53                      & 43.2               & 83.7                         & 74.2                          & 74.5 \\
        \textbf{Two-stage}    & 75.9                        & 82.9               & 55.2                    & 43.5               & 85.3                         & 74                            & 79.1                  \\
        \bottomrule
    \end{tabular}}
    \caption{Comparison between single-stage and two-stage training. }
    \label{tab:two_stage_training}
\end{table}

